Faster Algorithms for the Constrained k-means Problem

The classical center based clustering problems such as $k$-means/median/center assume that the optimal clusters satisfy the locality property that the points in the same cluster are close to each other. A number of clustering problems arise in machine learning where the optimal clusters do not follow such a locality property. Consider a variant of the $k$-means problem that may be regarded as a general version of such problems. Here, the optimal clusters $O_1, ..., O_k$ are an arbitrary partition of the dataset and the goal is to output $k$-centers $c_1, ..., c_k$ such that the objective function $\sum_{i=1}^{k} \sum_{x \in O_{i}} ||x - c_{i}||^2$ is minimized. It is not difficult to argue that any algorithm (without knowing the optimal clusters) that outputs a single set of $k$ centers, will not behave well as far as optimizing the above objective function is concerned. However, this does not rule out the existence of algorithms that output a list of such $k$ centers such that at least one of these $k$ centers behaves well. Given an error parameter $\varepsilon > 0$, let $\ell$ denote the size of the smallest list of $k$-centers such that at least one of the $k$-centers gives a $(1+\varepsilon)$ approximation w.r.t. the objective function above. In this paper, we show an upper bound on $\ell$ by giving a randomized algorithm that outputs a list of $2^{\tilde{O}(k/\varepsilon)}$ $k$-centers. We also give a closely matching lower bound of $2^{\tilde{\Omega}(k/\sqrt{\varepsilon})}$. Moreover, our algorithm runs in time $O \left(n d \cdot 2^{\tilde{O}(k/\varepsilon)} \right)$. This is a significant improvement over the previous result of Ding and Xu who gave an algorithm with running time $O \left(n d \cdot (\log{n})^{k} \cdot 2^{poly(k/\varepsilon)} \right)$ and output a list of size $O \left((\log{n})^k \cdot 2^{poly(k/\varepsilon)} \right)$.

==> finding-clusters.tex <==
\subsection{Finding the a good center from the list}
One important issue that we need to address is that the way we defined the constrained $k$-means problem, it was sufficient for any algorithm to output a list of elements, each element being a set of $k$ centers such that one of these set of $k$ centers is good.
However, the clustering task requires one to output one set of $k$ centers.
So, the question is -- how do we identify a good $k$ center from the list. That is, the one that gives the $(1+\veps)$ approximation to the objective function.
In general, this does not seem possible since the optimal target clustering which is an arbitrary partition of the dataset is not known.
However, if the target optimal clustering satisfies certain properties then identifying the ``best" $k$ center from the list might be possible.
That is, we do this in a problem specific manner. For the specific problem such as $r$-gather or capacitated clustering we give an algorithm to pick the best set of $k$ center from the list.
Ding and Xu~\cite{dx15} give such algorithms for various problems in the constrained setting.
We would like to encourage the reader to look at their paper for a comprehensive discussion.
For better readability, we just repeat some of these algorithms below.

\begin{itemize}
\item {\em $k$-means/median}: For instance, if the optimal cluster is a Voroni partition, as in the case of $k$-means and $k$-median, then we can pick the $k$ center that minimises the objective function
\footnote{Note that the Voronoi partition w.r.t. such a $k$ center might not be the target optimal clustering but still it gives a $(1+\veps)$-approximation}.

\item {\em $r$-gather $k$-means clustering}: The formal definition of the this problem is -- given a dataset $X \subseteq \mathbb{R}^d$, cluster $X$ into $k$ clusters such that each cluster has at least $r$ points and the sum of squared Euclidean distance of each of the points to the mean of its cluster is minimised. Let $\opt$ denote the optimal cost.
We will now see how to obtain a clustering $O = (O_1, ..., O_k)$ from the list $L$ of $k$ centers containing at least one good $k$ center such that $cost(O) \leq (1 + \veps) \cdot \opt$.
For each set of $k$ centers $\{c_1, ..., c_k\}$ in the list construct a flow network as shown in Figure.
The vertices in $P$ correspond to points in $X$ and vertices in $Q$ correspond to centers $\{c_1, ..., c_k\}$.
The cost of the edge from $x$ to $c_i$ is equal $||x - c_i||^2$.
The demand and capacity of $c_i$ is $r$ and $n$ respectively.
The clustering corresponding to $\{c_1, ..., c_k\}$ is the matching given by the solution of the minimum cost circulation problem on the flow network.
Finally, the clustering corresponding to the $k$ centers with minimum cost is produced.
Note that such a clustering indeed gives a $(1 + \veps)$ approximation.
\end{itemize}

\begin{figure}
\centering
\includegraphics[scale=0.3]{flow}
\caption{Flow network for obtaining the approximate clustering for the $r$-gather $k$-means clustering problem.}
\end{figure}

